Frequency Chirping of Energetic-Particle-Driven Geodesic Acoustic Modes in Tokamaks

A suprathermal population of ions is present in tokamak plasmas due to external heating mechanisms and fusion reactions. These energetic particles (EPs) can drive waves unstable, via inverse Landau damping. An example is the energetic-particle-induced geodesic acoustic mode (EGAMs). In this work, investigate the nonlinear dynamics of EGAMs by means of global gyrokinetic simulations with the particle-in-cell code ORB5. In particular, we study the nonlinear evolution of the frequency, known as "frequency chirping". To investigate the underlying phase-space dynamics, Phase Space Zonal Structure (PSZS) diagnostics are employed. By identifying the resonance energy from the phase-space distribution and reconstructing the corresponding mode frequency, an independent estimate of the frequency evolution is obtained. The reconstructed frequencies show good agreement with those extracted directly from continuous wavelet transform analysis of the electric-field signal, establishing a direct correspondence between observable frequency chirping and the nonlinear evolution of resonant energetic particles in phase space.

==> part2.tex <==
%====================== Part 2 ======================
% Theoretical Background

\section{Theoretical Background}

\subsection{Geodesic Acoustic Modes}

GAMs are axisymmetric oscillations of the zonal
$\vb{E}\times\vb{B}$ flow, whose restoring force originates from the geodesic curvature
of the magnetic field \cite{winsor1968}. When a flux-surface-averaged radial electric field perturbation
is generated, the associated $\vb{E}\times\vb{B}$ flow induces a compression of the
plasma density on the flux surface. The resulting density perturbation drives parallel
currents, which react back on the radial electric field, forming a closed feedback loop
that sustains oscillatory dynamics.

In thermal plasmas, GAMs oscillate at an acoustic frequency of order
\begin{equation}
\omega_{\mathrm{GAM}} =
\frac{\sqrt{2}\, c_s}{R_0},
\label{eq:omega_gam}
\end{equation}
where $c_s$ is the ion sound speed and $R_0$ is the major radius of the tokamak.
Kinetic effects, in particular ion Landau damping, lead to strong attenuation of GAMs
in Maxwellian plasmas.

\subsection{Energetic-Particle-Driven GAMs}

When energetic particles (EPs) are present, the dynamics change qualitatively. Non- Maxwellian EP velocity distributions, such as the double bump-on-tail profiles, can provide a positive velocity-space gradient near resonance, enabling energy transfer from particles to the wave through inverse Landau damping. Consequently, GAMs can become unstable, giving rise to EGAMs \cite{biancalani2017}. In nonlinear simulations, the growth is eventually arrested and the mode saturates at a finite amplitude; the saturation physics is discussed in Sec. 4.


